Can You Improve My Code? Optimizing Programs with Local Search

This paper introduces a local search method for improving an existing program with respect to a measurable objective. Program Optimization with Locally Improving Search (POLIS) exploits the structure of a program, defined by its lines. POLIS improves a single line of the program while keeping the remaining lines fixed, using existing brute-force synthesis algorithms, and continues iterating until it is unable to improve the program's performance. POLIS was evaluated with a 27-person user study, where participants wrote programs attempting to maximize the score of two single-agent games: Lunar Lander and Highway. POLIS was able to substantially improve the participants' programs with respect to the game scores. A proof-of-concept demonstration on existing Stack Overflow code measures applicability in real-world problems. These results suggest that POLIS could be used as a helpful programming assistant for programming problems with measurable objectives.

==> algos/probe.tex <==
\begin{algorithm}[t]
    \caption{--Fatemeh--PROBE}
    \label{probe}
    \KwData{$h$, $id$, $t_{probe}$, $HList$, PCFG}
    \KwResult{$best\_program$}
    $PCFG \gets {Uniform Distribution}$\;
    $p_{init} \gets$ \FuncCall{GetProgram}{$id$}\;
    $PCFG.$\FuncCall{Init}{$p_{init}$}\;\label{probe:init}
    $all\_candidates \gets Priority Queue(size = 20)$\;\label{probe:queue}
    $update\_freq \gets 20$\;\label{probe:updateinit}
    $best\_p \gets p_{init}$\;
    \While{\FuncCall{IfTimeRemains}{$t_{probe}$}}{
    $PCFG\_cand \gets [ ]$\;
    $plist \gets [p_{init}, \text{all terminals in DSL}]$\;
    $outputs \gets set()$\;
    \For{cost from 1 to 100}{
    \For{p in \FuncCall{Grow}{$PCFG, outputs, p$, cost}}{
      $h_{new} \gets$ \FuncCall{ModifyFunction}{$id, p$}\;\label{probe:modify}
      $h_{new}.$ \FuncCall{BayesOpt}{$h_{new},id, HList$}\;\label{probe:bayes}
      $score \gets$ \FuncCall{SimRate}{$h, i, HList$}\;\label{probe:DQN}
      $p \gets$ \FuncCall{GetProgram}{$id$}\;
      $all\_candidate$.\FuncCall{push}{$(score, p)$}\;
      \If{p is in $all\_candidates$}{
      $PCFG\_cand$.\FuncCall{add}{(s,p)}\;
      \If{\FuncCall{Eval}{$h$,$p$} > \FuncCall{Eval}{$h$,$best\_p$}}{$best\_p \gets p$}\label{probe:eval}
      \If{$update\_freq == len(PCFG\_cand)$}{
      PCFG.\FuncCall{Update}{$PCFG\_cand$}\;
      $update\_freq$.\FuncCall{Update}{}\;\label{probe:updateupdate}
      $PCFG\_cand \gets [ ]$\;
      break\;
      }
      }\label{probe:update}
      }\label{probe:grow}
      }\label{probe:cost}
    }
\end{algorithm}
